Optimal Infinite Horizon Decentralized Networked Controllers with Unreliable Communication

We consider a decentralized networked control system (DNCS) consisting of a remote controller and a collection of linear plants, each associated with a local controller. Each local controller directly observes the state of its co-located plant and can inform the remote controller of the plant's state through an unreliable uplink channel. The downlink channels from the remote controller to local controllers were assumed to be perfect. The objective of the local controllers and the remote controller is to cooperatively minimize the infinite horizon time average of expected quadratic cost. The finite horizon version of this problem was solved in our prior work [2]. The optimal strategies in the finite horizon case were shown to be characterized by coupled Riccati recursions. In this paper, we show that if the link failure probabilities are below certain critical thresholds, then the coupled Riccati recursions of the finite horizon solution reach a steady state and the corresponding decentralized strategies are optimal. Above these thresholds, we show that no strategy can achieve finite cost. We exploit a connection between our DNCS Riccati recursions and the coupled Riccati recursions of an auxiliary Markov jump linear system to obtain our results. Our main results in Theorems 1 and 2 explicitly identify the critical thresholds for the link failure probabilities and the optimal decentralized control strategies when all link failure probabilities are below their thresholds.

==> approach.tex <==


\subsection{Summary of the Approach}

Previous sections provide optimal controllers for certain infinite horizon DNCS problems.
The key idea is to construct an auxiliary MJLS and use MJLS properties to extend optimal controllers in finite horizons to their counterparts in the infinite horizon.
This approach of solving an infinite horizon DNCS problem can be summarized as the following main steps:
\begin{enumerate}
%\item Identify the set of modes $\mathcal M = \{1,2,\dots,M\}$ of the DNCS from its (randomized) information structures.
\item Solve the finite horizon version of the DNCS problem and obtain matrices $P_t^m, m \in \mathcal M = \{1,2,\dots,M\}$ which satisfy $M$ coupled Ricatti recursions 
\begin{align}
P_t^m =  \Omega(\sum_{j} \theta^{mj} P_{t+1}^j,Q^m,R^m,A^m,B^m)
\label{eq:P_finite_general}
\end{align}
for some matrices $Q^m,R^m,A^m,B^m$ and positive numbers $\theta^{mj}$ for $m,j \in\mathcal M$. Note that we can scale the $\theta$'s such that $\sum_{j\in\mathcal M}\theta^{mj} = 1$ by appropriately scaling $A^m$ and $R^m$ for all $m\in\mathcal M$.


\item Construct a $M$-mode auxiliary MJLS with transition probabilities $\theta^{mj}$ and system matrices $Q^m,R^m,A^m,B^m$
based on the Ricatti recursions \eqref{eq:P_finite_general}.


\item Analyze stability criteria of the auxiliary MJLS which directly translate to stability conditions for the DNCS.

\item When the auxiliary MJLS is stable, solve its associated DCARE to obtain optimal strategies for the infinite horizon DNCS problem.
\end{enumerate}


\subsection{The Information Switching}
Even though the auxiliary MJLS is an artificial system without physical meanings (See Remark ?), the connection between a DNCS and a MJLS provides a general method to analyze switching behaviors of a DNCS. 
In particular, a DNCS with delays and packet-drop channels can be viewed as a decentralized control problem with a randomized information structure \cite{RPN}.
In other words, a DNCS can be viewed as a special class of ``switched" systems where each controller's information is switching between different structures or patterns. 

The information of the remote controller in Section \ref{sec:model_2_controllers} switches between two structures: no observation when the packet is dropped, and perfect observation when the transmission is successful.
For this two-controller DNCS, each information structure of the remote controller can be treated as a ``mode". Consequently, the closed-loop system under the optimal strategies become a two-mode switching system.
It is worth noting that, even though the DNCS can be thought of as a two-mode switching system, it cannot be modled by an MJLS due to its decentralized information.
The auxiliary MJLS is an artificial two-mode system constructed to help analyze the behavior of the DNCS with two switching information structures.

In the $(N+1)$-controller DNCS presented in Section \ref{sec:model_N_controllers}, 
the remote controller's information about each of the $N$ subsystem switches between two patterns: knowing $X^n_t$ or not. 
Therefore, its information is switching among $2^N$ structures.
The analysis of these information structures can be simplified from the decoupled dynamics.
In fact, the remote controller's information about each of the $N$ subsystems depends only on the $n$th link because the subsystems' states are conditional independent. Consequently, we construct an auxiliary $(N+1)$-mode MJLS where mode $0$ corresponds to the perfect information case, and each of the other $N$ modes corresponds to the failure of each of the $N$ links.


%In this section, we present a high-level description of the approach we used to solve Problem \ref{problem_infinite_2C}. We will then illustrate how this methodology can used to solve the extension of the system model of Section \ref{sec:model_2_controllers} to the case where instead of 1 local controller, we have $N$ local controllers. 
%
%
%Consider a general DNCS consisting of $N$ subsystems where each subsystem is affiliated with a controller. Subsystem $i$'s dynamics are given by
%\begin{align}
%X_{t+1}^i = & \sum_{j=1}^N \Big( A^{ij} X_t^j +  B^{ij} U^j_t \Big) + W_t^i
% \label{Model:system_general}
%\end{align}
%for $i = 1,2,\dots,N$.
%At each time $t$, $X_t^i$ is the state and $W_t^i$ is the noise of subsystem $i$. $U_t^i$ is the control of controller $i$, and $A^{ij}, B^{ij}$ are matrices with appropriate dimensions for all $i,j = 1,\dots,N$.
%
%
%Each controller can perfectly observes the state of its subsystem, and the controllers can communicated with each other through unreliable communication links.
%Let $\Gamma_t^{ij}$ be a Bernoulli random variable describing the state of the link from controller $i$ to controller $j$ ($1$ is active and $0$ is broken).
%Let $Z_t^{ij}$ be the message received by controller $i$ from controller $i$ so that 
%$Z_t^{ij} = X^j_t$ if $\Gamma_t^{ij} = 1$ and $Z_t^{ij} = \emptyset$ if $\Gamma_t^{ij} = 0$.
%Depending on the transmission protocols, each controller $i$'s information at time $t$ is denoted by $H^i_t$ where 
%$H^i_t$ is a subset of $X^i_{0:t},  Z_{0:t}^{ij}$.
%%Let $\mathcal{H}^i_t$ be the spaces of all possible realizations of $H^i_t$
%Then a control strategy $g^i=(g^i_{0},g^i_1,\dots,g^i_{t},\dots)$ is a collection of measurable mappings such that $U^i_t = g^i_t(H^i_t)$.
%Let $\mathcal{G}$ denote the set of all possible control strategies $g = (g^1,\dots,g^N)$ of the controllers that ensure that all states and control actions have finite second moments.
%
%Consider the quadratic instantaneous cost $c(X_t,U_t) = X_t^\tp Q X_t + U_t^\tp R U_t$ 
%where $Q$ is a PSD matrix, and $R$ is a PD matrix.
%Then the performance of DNCS control strategies $g$ over a finite horizon $T$ is measured by the total expected cost:
%\begin{align}
%J_T(g):=\ee^{g}\left[\sum_{t=0}^T c(X_t,U_t)\right].
%\label{Model:J_T_general}
%\end{align}
%
%For this general DNCS, we can consider the finite horizon and infinite horizon optimal control problems defined as follows
%\begin{problem}[Finite Horizon general DNCS Optimal Control]
%\label{problem_finite_general}
%For the general DNCS described described above, solve the following finite horizon strategy optimization problem:
%\begin{align}
%\inf_{g \in\mathcal{G}} 
%J_T(g)
%\label{Model:obj_finite_general}
%\end{align}
%\end{problem}
%\begin{problem}[Infinite Horizon general DNCS Optimal Control]
%\label{problem_infinite_general}
%For the general DNCS described described above, solve the following infinite horizon  strategy optimization problem:
%\begin{align}
%&\inf_{g \in\mathcal{G}} 
%J_{\infty}(g)
%:= \inf_{g \in\mathcal{G}} 
%\limsup_{T\rightarrow\infty} \frac{1}{T+1} J_{T}(g).
%\label{Model:obj_infinite_general}
%\end{align}
%
%\end{problem}
%
%
%Suppose that we have the solution to the finite horizon Problem \ref{problem_finite_general} and the solution depends on $M$ matrices $P_t^m, m \in \mathcal M = \{1,2,\dots,M\}$ that satisfy
%\begin{align}
%P_t^m =  \Omega(\sum_{j} \theta^{mj} P_{t+1}^j,Q^m,R^m,A^m,B^m)
%\label{eq:P_finite_general}
%\end{align}
%for some matrices $Q^m,R^m,A^m,B^m$ and positive numbers $\theta^{mj}$ for $m,j \in\mathcal M$. Note that we can scale the $\theta$'s such that $\sum_{j\in\mathcal M}\theta^{mj} = 1$ by appropriately scaling $A^m$ and $R^m$ for all $m\in\mathcal M$.
%
%\red{Think about if we can have a general structure and can prove the connection from finite horizon to infinite horizon.}
%\red{One possible way: suppose the optimal cost of the finite horizon problem is given by
%\begin{align}
%\sum_{t=1}^T \mathcal L(P_t^1,P_t^2,\dots,P_t^M)
%\end{align}
%where $\mathcal L$ is a function of the matrices such that $\mathcal L(P_t^1,P_t^2,\dots,P_t^M) \rightarrow \infty$ when $P_t^m \rightarrow \infty$ for any $m$.
%}
%
%Given the above finite horizon optimal strategies, the approach to solve the infinite horizon Problem \ref{problem_infinite_general} is to construct an auxiliary MJLS: 
%\begin{itemize}
%\item The $A^{MJ}(m), B^{MJ}(m)$ matrices in the dynamics \eqref{eq:MJ_X} are $A^m,B^m$.
%\item The mode transition matrix in \eqref{eq:MJ_M} is given by $\theta^{mj}$ for $m,j \in\mathcal M$.
%\item The matrices $Q^{MJ}(m), R^{MJ}(m)$ of the cost function \eqref{eq:MJ_c} are given by $Q^m,R^m$.
%\item The initial probability distributions $\pi_{X_0^{MJ}}$ and $\pi_{M_0}$ are such that  $X^{MJ}_0 = 0$ and $M_0 = 1$.
%\end{itemize}
%
%Then the optimal strategies of the infinite horizon problem can be obtained by solving the DCARE of the auxiliary MJLS, and the stability of the general DNCS is determined by the stability of this auxiliary MJLS.
%
%
%The main steps of the our approach to solve the infinite horizon Problem \ref{problem_infinite_general} can be summarized as follows:
%\begin{enumerate}
%\item Solve the finite horizon version Problem \ref{problem_finite_general} and identify the matrices $P_t^m, m \in \mathcal M = \{1,2,\dots,M\}$ and their Ricatti recursions \eqref{eq:P_finite_general}.
%
%\item Construct an auxiliary MJLS based on the Ricatti recursions \eqref{eq:P_finite_general}.
%
%\item Analyze the stability of the auxiliary MJLS and Solve its associated DCARE to obtain the optimal strategies for the general DNCS infinite horizon optimal control Problem \ref{problem_infinite_general}.
%\end{enumerate}

==> conclusion.tex <==
We considered a networked control system (NCS) consisting of a remote controller and a collection of linear plants, each
associated with a local controller. Each local controller directly observes the state of its co-located plant and can inform the remote controller of the plant’s state through an unreliable uplink channel. The downlink channels from the remote controller to
local controllers are assumed to be perfect. The objective of the local controllers and the remote controller is to cooperatively
minimize a quadratic performance cost. The finite horizon version of this problem was solved in our prior work \cite{asghari_optimal_2017_arXiv}. The optimal strategies in the finite horizon case were shown to be characterized by coupled Riccati recursions.  In this paper, we showed that the finite horizon solution is related to  the solution of a centralized control problem for an auxiliary Markov jump linear system. By exploiting this connection, we investigated the infinite horizon decentralized control problem. Our main result in Theorem \ref{thm:DC_infinite} characterizes a set of critical thresholds $p_c^n$, one for each link failure probability $p^n$. We showed that no decentralized control strategies can give finite cost for the DNCS if one of the link failure probabilities is above the threshold. Further, when all link failure probabilities are below the thresholds, Theorem \ref{thm:DC_infinite} provides an explicit characterization of the optimal strategies.

==> model.tex <==
In this section, we extend the system model of Section \ref{sec:model_2_controllers} to the case where instead of 1 local controller, we have $N$ local controllers, $C^1,C^2, \ldots,C^N$, each associated to a co-located plant as 
%Consider a discrete-time system with $N$ plants, $N$ local controllers, $C^1,C^2, \ldots,C^N$, and one remote controller $C^0$ as 
shown in Fig. \ref{fig:SystemModel}. We use $\mathcal{N}$ to denote the set $\{1,2, \ldots, N\}$ and $\overline{\mathcal{N}}$ to denote $\{0,1,\ldots, N\}$.
The linear dynamics of plant $n \in \mathcal{N}$ are given by
\begin{align}
&X_{t+1}^n \!=\! A^{nn} X_t^n + B^{nn}U^{n}_t+ B^{n0} U^0_t + W_t^n, t=0,\dots,T,
 \label{Model:system}
\end{align}
where $X_t^n\in \R^{d_X^n}$ is the state of the plant $n \in \mathcal{N}$ at time $t$,
$U^n_t \in \R^{d_U^n}$ is the control action of the controller $C^{n}$, $n \in {\color{black} \overline{\mathcal{N}}}$, and $A^{nn}, B^{nn}, B^{n0}$, $n \in \mathcal{N}$, are matrices with appropriate dimensions.
We assume that $X^n_0 = 0$, $W^n_t$, $n \in \mathcal{N}$ and $t \geq 0$, are i.i.d noise processes with zero mean and $\cov(W_t^n) = \mathbf{I}$. Note that we do not assume that $W_{t}^{n}$, $n \in \mathcal{N}$ and $t \geq 0$, are Gaussian.

The overall dynamics can be written as
\begin{align}
X_{t+1} = A X_t + BU_t + W_t
\label{overall_state_dynamic}
\end{align}
where $X_t = \vecc(X^{1:N}_t), U_t = \vecc(U^{0:N}_t),W_t = \vecc(W^{0:N}_t)$ and $A,B$ are defined as

\begin{align}
A &= \begin{bmatrix}
   A^{11} & & \text{\huge0}\\
          & \ddots & \\
     \text{\huge0} & & A^{NN}
\end{bmatrix}, 
B= 
\begin{bmatrix}
B^{10} &  B^{11} & & \text{\huge0}\\
\vdots     &     & \ddots & \\
B^{N0}  &   \text{\huge0} & & B^{NN}
\end{bmatrix}.
\label{eq:thm_matricesABB}
\end{align}

\begin{singlespace}

\input{system_model}
\end{singlespace}
\input{timeline}

\subsubsection*{Communication Model}
\label{subs:comm_model}
We assume that the communication network between the local controller $C^{n}$, $n \in \mathcal{N}$, and the remote controller $C^0$ is the same as one described for the local controller $C^{1}$ is Section \ref{subs:comm_model_2C}. In particular, there exists an unreliable channel with link failure probability $p^n$ from the local controller $C^{n}$, $n \in \mathcal{N}$, to the remote controller $C^0$, through which the local controller $C^{n}$ sends the perfectly observed state  $X_t^n$ of its co-located plant. The state of this channel at time $t$ is described by Bernoulli random variable $\Gamma_t^n=0$ and the output of this channel at time $t$ is denoted by $Z_t^n$ where $\Gamma_t^n$ and $Z_t^n$ are described similar to \eqref{Model:channel_2C}.

%At each time $t$ the local controller $C^{n}$, $n \in \mathcal{N}$, perfectly observes the state $X^n_t$ and sends the observed state to the remote controller $C^0$ through an unreliable channel with link failure probability $p^n$. 
%Let $\Gamma_t^n$ be a Bernoulli random variable describing the state of this channel with $\Gamma_t^n=0$ when the link is broken and $\Gamma_t^n=1$ otherwise.
%We assume that $\Gamma_{t}^{1:N}$, $t \geq 0$, are independent random variables and they are independent of $W_{0:t}^{1:N}$, $t \geq 0$.
%Furthermore, let $Z_t^n$ be the output of the channel between the local controller $C^{n}$ and the remote controller $C^0$ at time $t$. Thus, we have
% \begin{align}
%\Gamma_t^n = &\left\{\begin{array}{ll}
%1 & \text{ with probability }(1-p^n),\\
%0 & \text{ with probability }p^n.
%\end{array}\right.
%\\
%Z_t^n = &
%\left\{\begin{array}{ll}
%X_t^n & \text{ when } \Gamma_t^n = 1,\\
%\emptyset & \text{ when } \Gamma_t^n = 0.
%\end{array}\right.
%\label{Model:channel}
%\end{align}
Unlike the unreliable uplinks, we assume that there exist perfect links from $C^0$ to $C^{n}$, for $n \in \mathcal{N}$. Therefore, $C^0$ can share $Z_t^{1:N}$ and $U_{t-1}^0$ with all local controllers $C^{1:N}$.
All controllers select their control actions at time $t$ after observing $Z_t^{1:N}$. 
A schematic of the time ordering of  variables is shown in Fig. \ref{fig:timing}. 
We assume that for all $n \in \mathcal{N}$, the links from controllers $C^{n}$ and $C^0$ to the plant $n$ are perfect.

%At each time $t$, the remote controller chooses its control action $U^R_t$ after receiving $Z_t$, and 
%the local controller chooses its control action $U^L_t$ after the reception of $Z_t$ from the ACK packet.

\subsubsection*{Information structure and cost}
\label{subs:info_cost_2C}
Let $H^{n}_t$ denote the information available to controller $C^{n}$, $n \in {\color{black} \overline{\mathcal{N}}}$, to make decisions at time $t$. %\footnote{$U^R_{t-1}$ is not directly observed by $C^{L^n}$ at time $t$, but $C^{L^n}$ can obtain $U^R_{t-1}$ because $U^R_{t-1}=g^R_t(H^R_{t-1})$ and $H^R_{t-1} \subset H^{L^n}_{t}$. } 
Then,
\begin{align}
H^{n}_t&= \{X^n_{0:t}, U^{n}_{0:t-1}, Z_{0:t}^{1:N}, U^0_{0:t-1}\}, \hspace{2mm} n \in \mathcal{N} \notag \\
H^0_t &= \{Z_{0:t}^{1:N}, U^0_{0:t-1}\}. 
\label{Model:info}
\end{align}
%Note that $Z_t$ is included in the information of local controller at time $t$ because the local controller chooses its control action after receiption of ACK packet from the remote controller. Furthermore, $Z_t$ is included in the information of remote controller at time $t$ because the remote controller chooses its control action after receiption of $Z_t$.
Let $\mathcal{H}^{n}_t$ be the space of all possible realizations of $H_t^n$.
Then, $C^{n}$'s actions are selected according to
\begin{align}
U^{n}_t &= g^{n}_t(H^{n}_t), \hspace{2mm}  n \in {\color{black} \overline{\mathcal{N}}},
\label{Model:strategy}
\end{align}
where $g^{n}_t:\mathcal{H}^{n}_t{\color{black} \to } \R^{d_U^n}$ is a Borel measurable mapping.
We use $g:=(g^0_{0},g^0_1,\dots,g^1_{0},g^1_1,\dots, g^N_{0},g^N_1,\dots,)$ to denote the control strategies of $C^0$ and $C^{1:N}$.
%The collection of mappings $g_0^n, \ldots, g_T^n$ is called the strategy of  controller $C^n$ and is denoted by $g^n$. The collection of all controllers' strategies, $g^{0:N}$, is called the strategy profile\footnote{When it is clear from the context, we will simply use $g$ instead of $g^{0:N}$.}. 
%We denote the space of all Borel measurable functions $g^{L^n}_t$ and $g^R_t$ by $\mathcal{G}^{L^n}_t$ and $\mathcal{G}^R_t$, respectively.
%Let $\mathcal{G}^{L^n}_t$ and $\mathcal{G}^R_t$ denote the set of all possible control strategies  $g^{L^n}_t$ and $g^R_t$, respectively.
% that ensure all random variables (state and control actions) have finite second moments.

The instantaneous cost $c_t(X_t, U_t)$ of the system is a quadratic function similar to the one described in \eqref{Model:cost_2C} where $X_t = \vecc(X^{1:N}_t), U_t = \vecc(U^{0:N}_t)$ and 
%
%given by
%\begin{align}
%&c_t(X_t^{1:N}, U^{0:N}_t) = 
%X_t^{\tp} Q X_t + U_t^{\tp} R U_t
%\label{cost_function}
%\end{align}
%where
\begin{align}
Q= \begin{bmatrix}
Q^{11} &\ldots &Q^{1N} \\
\vdots & \ddots & \vdots \\
Q^{N1} & \ldots & Q^{NN}
\end{bmatrix}, R= \begin{bmatrix}
R^{00} &R^{01} &\ldots &R^{0N} \\
R^{10} &R^{11} &\ldots &R^{1N} \\
\vdots &\vdots & \ddots & \vdots \\
R^{N0}  & \ldots & \ldots & R^{NN} 
\end{bmatrix}.
\label{matrix_structure}
\end{align}
$Q$ is a symmetric positive semi-definite (PSD) matrix and $R$ is a symmetric positive definite (PD) matrix. 

\subsubsection*{Problem Formulation}
\label{subs:prob_formulaiton}
Let $\mathcal{G}$ denote the set of all possible control strategies of $C^{0:N}$ that ensure that all states and control actions have finite second moments. The performance of control strategies $g$ over a finite horizon $T$ is measured by $J_T(g)$ described in \eqref{Model:J_T_2C}.

We refer to the system described above as the \emph{decentralized networked control system} with $N$ Local controller and 1 Remote controller (NL1R-DNCS).
We consider the problem of strategy optimization  for the NL1R-DNCS over finite  and infinite time horizons. These two problems are formally defined below.
\begin{problem}
\label{problem_finite}
For the NL1R-DNCS described above, %determine decentralized control strategies $g$ that optimize the  total expected cost over a finite horizon of duration $T$. In other words, 
solve the following strategy optimization problem:
\begin{align}
\inf_{g \in\mathcal{G}} 
J_T(g)
\label{Model:obj_finite}
\end{align}
\end{problem}


\begin{problem}
\label{problem_infinite}
For the NL1R-DNCS described above, %by \eqref{Model:system}-\eqref{matrix_structure}, find decentralized strategies $g$ that minimize the  infinite horizon average cost.  In other words, 
solve the following strategy optimization problem:
\begin{align}
&\inf_{g \in\mathcal{G}} 
J_{\infty}(g)
:= \inf_{g \in\mathcal{G}} 
\limsup_{T\rightarrow\infty} \frac{1}{T+1} J_{T}(g).
\label{Model:obj_infinite}
\end{align}

\end{problem}

==> old_proof_claim1_EDITED.tex <==
\section{Proof of Claim \ref{claim:cost_optimal_2C}}
\label{proof_claim:cost_optimal_2C}

\blue{Partially Edited OLD proof}

In order to show that \eqref{eq:costforgstar_2C} holds, it suffices to show that the following equation is true for all $t \geq 0$:
\begin{align}
\ee^{g*} [ c(X_t,U_t^*) | H_t^0]=  \tr(\Lambda_*)  + \ee^{g*} [V_t - V_{t+1} | H_t^0],
\label{main_goal_2C}
\end{align}
\blue{where $U^*_t$ are the control actions at time $t$ under $g^*$.
This is because by taking the expectation of \eqref{main_goal_2C} and summing it from $t=0$ to $T$, we obtain}
\begin{align}
J_{T}(g^*) 
= & \sum_{t=0}^T \ee^{g*} [ c(X_t,U_t^*) ]
\notag\\
=&(T+1) \tr(\Lambda_*) 
+ \ee^{g*} [V_0 - V_{T+1} ]
\notag\\
=&(T+1) \tr(\Lambda_*) 
- \ee^{g*} [V_{T+1} ],
\end{align}
where the last equality holds because $V_0 = 0$ (recall that $X_0 = \hat X_0 =0$). 

%We want to show that \eqref{eq:costforgstar_2C} holds. To this end, we show that 
%\begin{align}
%\ee [ c(X_t,U_t^*) | H_t^0]=  \tr(\Lambda_*)  + \ee [V_t - V_{t+1} | H_t^0].
%\label{main_goal_2C}
%\end{align}
%where $\Lambda_*=(1-p^1) P_{*}^0+p^1 P_{*}^1$.
%Then, taking the expectation of the above equation and summing it from $0$ to $T$, the correctness of \eqref{eq:costforgstar_2C} is concluded as follows,
%\begin{align}
%J_{T}(g^*) 
%= & \sum_{t=0}^T \ee [ c(X_t,U_t^*) ]
%\notag\\
%=&(T+1) \tr(\Lambda_*) 
%+ \ee [V_0 - V_{T+1} ]
%\notag\\
%=&(T+1) \tr(\Lambda_*) 
%- \ee [V_{T+1} ],
%\end{align}
%where the last equality holds because $V_0 = 0$. 

Now, to show that \eqref{main_goal_2C} holds, \blue{first note that $\ee^{g*}[V_t | H_t^0] = V_t$ since $V_t$, given by \eqref{V_t_2C}, is a function of $H^0_t$}.  Hence, \eqref{main_goal_2C} is equivalent to
\begin{align}
\ee^{g*} [ c(X_t,U_t^*) | H_t^0] + \ee^{g*} [ V_{t+1} | H_t^0] = \tr(\Lambda_*)  + V_t. \label{eq:main_goal_2C_2}
\end{align}
 In the following subsections we will calculate $\ee^{g*} [ c(X_t,U_t^*) | H_t^0]$ and $\ee^{g*}[V_{t+1} | H_t^0]$.  To do so, we define 
\begin{align}
&\hat X_{t+1|t} := \ee [X_{t+1}|H^0_{t}]
\\
&\Sigma_{t+1|t} := \cov(X_{t+1}|H^0_{t})
 \\
&\Sigma_t := \cov(X_{t}|H^0_{t}),
\label{Sigma_2C}
\end{align}
and recall that $\hat{X}_t = \ee [X_{t}|H^0_{t}]$.

\subsection{Calculating $\ee^{g*} [ c(X_t,U_t^*) | H_t^0]$}
Note that 
\begin{small}
\begin{align}
&\ee^{g*} [ c(X_t,U_t^*) | H_t^0]=  \underbrace{\ee^{g*} [X_t^\tp Q X_t | H_t^0]}_{\mathbb{T}_4} + \underbrace{\ee^{g*}[U_t^{*\tp} R U_t^* | H_t^0]}_{\mathbb{T}_5}. 
\label{cost_given_h_2C}
\end{align}
\end{small}
We can simplify the term $\mathbb{T}_4$ as follows
\begin{small}
\begin{align}
\mathbb{T}_4 &=  \hat X_t^\tp Q\hat X_t + \ee^{g*} \Big[(X_t-\hat X_t)^\tp Q (X_t-\hat X_t)|H^0_t\Big] \notag \\
& =  \hat X_t^\tp Q\hat X_t + \tr\big(Q\Sigma_t \big)
=  \hat X_t^\tp Q^{\diamond}(0)\hat X_t + \tr\big(Q^{\diamond}(1)\Sigma_t \big), \label{eq:T4eq}
\end{align}
\end{small}
where the last equality is correct because from \eqref{eq:MJLS_Q}, $Q^{\diamond}(0) = Q^{\diamond}(1) = Q$. 

 From \eqref{eq:opt_U_2C_fixed}, we have $U_t^* = K_*^0\hat X_t + \tilde K_*^1 (X_t - \hat X_t)$, where $\tilde K_*^1 =  \bmat{\mathbf{0} \\ K_*^1 }$.  Therefore, we can simplify the term $\mathbb{T}_5$ as follows
\begin{small}
\begin{align}
\mathbb{T}_5 &= (K_*^0\hat X_t)^\tp R K_*^0\hat X_t \notag \\
& + \ee^{g*} \Big[(X_t-\hat X_t)^\tp (\tilde K_*^1)^{\tp} R \tilde K_*^1 (X_t-\hat X_t)|H^0_t\Big]
\notag\\
&= (K_*^0\hat X_t)^\tp R^{\diamond}(0) K_*^0\hat X_t + \tr \big( (\tilde K_*^1)^\tp R^{\diamond}(1) \tilde K_*^1 \Sigma_t \big),
 \label{cost_on_U_t_2C}
\end{align}
\end{small}
where the last equality is correct from definition of $R^{\diamond}(0), R^{\diamond}(1)$ in \eqref{eq:MJLS_R}.

Putting \eqref{cost_given_h_2C}, \eqref{eq:T4eq} and \eqref{cost_on_U_t_2C} together, we can write 
\begin{align}\label{eq:calculated_c}
&\ee^{g*} [ c(X_t,U_t^*) | H_t^0]=\underbrace{[ \hat X_t^\tp Q(0)\hat X_t +\tr(Q(1) \Sigma_t)]}_{=\mathbb{T}_4} \notag \\
&+ \underbrace{[(K_*^0\hat X_t)^\tp R(0) K_*^0\hat X_t + \tr( (\tilde K_*^1)^\tp R(1) \tilde K_*^1 \Sigma_t)]}_{=\mathbb{T}_5}.
\end{align}
\subsection{Calculating $\ee^{g*}[V_{t+1}|H^0_t]$}

\red{Start here}
From the definition of $V_{t+1}$ (see \eqref{V_t_2C})  we have
\vspace{-2mm}
\begin{small}
\begin{align}
& \ee^{g*}[V_{t+1}|H^0_t]= \underbrace{\ee^{g*}\Big[
\hat X_{t+1}^\tp P_*^0 \hat X_{t+1} \Big| H^0_t
\Big]}_{\mathbb{T}_6} + \underbrace{\ee^{g*}\Big[
\tr \big(P_*^{1} \Sigma_{t+1} \big) \Big| H^0_t \Big]}_{\mathbb{T}_7}.\label{eq:T6T7}
\end{align}
\end{small}
Note that if $\Gamma_{t+1} = 1$ (i.e., the link is active) $\hat X_{t+1} = X_{t+1}$ and   $\Sigma_{t+1} = 0$  and if $\Gamma_{t+1} = 0$ $\hat X_{t+1} = \hat X_{t+1|t}$ and $\Sigma_{t+1} = \Sigma_{t+1|t}$. That is, 
\red{Do the above statements need some justification? FYI Something is weird about 109 in the finite horizon paper}
\begin{align}
\label{estimation_state_2C}
&\hat X_{t+1} = \Gamma_{t+1}X_{t+1} +(1-\Gamma_{t+1}) \hat X_{t+1|t},  \\
 &\Sigma_{t+1}  = (1-\Gamma_{t+1}) \Sigma_{t+1|t}.
\label{estimation_covariance_2C}
\end{align}
Now, we use \eqref{estimation_state_2C} and \eqref{estimation_covariance_2C} to calculate  the terms $\mathbb{T}_6$ and $\mathbb{T}_7$ in \eqref{eq:T6T7}.

Note that from \eqref{estimation_state_2C}, $\hat X_{t+1}$ is equal to $\hat X_{t+1|t} + \Gamma_{t+1}(X_{t+1} -\hat X_{t+1|t})$. Therefore,  $\mathbb{T}_6$ can be written as
\vspace{-2mm}
\begin{small}
\begin{align}
&\mathbb{T}_6= 
\ee^{g^*}\Big[
\hat X_{t+1|t} ^\tp P_*^0 \hat X_{t+1|t} \Big| H^0_t \Big] \notag \\
&+ \ee^{g^*}\Big[
(X_{t+1} -\hat X_{t+1|t})^\tp \Gamma_{t+1} P_*^0 \Gamma_{t+1}(X_{t+1} -\hat X_{t+1|t}) \Big| H^0_t \Big] \notag \\ & = 
\hat X_{t+1|t} ^\tp P_*^0 \hat X_{t+1|t}+ (1-p^1) \tr (P_*^0 \Sigma_{t+1|t}).
\label{T_4_1}
\end{align}
\end{small}
Furthermore, using \eqref{estimation_covariance_2C}, it is straightforward to see that 
\vspace{-2mm}
\begin{small}
\begin{align}
&\mathbb{T}_7
= p^1 \tr (P_*^1  \Sigma_{t+1|t}).
\end{align}
\end{small}

In the subsequent analysis, we will make use of the following definitions and lemmas.
\begin{definition}\label{def:Pi_2}
Let $P_*$ denote the set of matrices $\{P^0_*,P^*_1\}$.  For $n=0,1$, we define
 \begin{align}
\Pi (P_*, n) := \sum_{m=0}^1 \theta^{nm} P_*^m,
\label{Pi_2_matrix}
\end{align}
where $\theta^{nm}$ are the mode transition probabilities  given in \eqref{eq:MJLS_theta}. We further define, for $n=0,1$,
\begin{align}
&\Omega^{\diamond}(P_*,n) := \Omega\big(\Pi(Y, n),Q^{\diamond}(n),R^{\diamond}(n),A^{\diamond}(n),B^{\diamond}(n) \big),
\label{Omega_MJ}
\\
&\Psi^{\diamond}(P_*,n) := \Psi \big(\Pi(Y, n),R^{\diamond}(n),A^{\diamond}(n),B^{\diamond}(n) \big),
\label{Psi_MJ}
\end{align}
where $\Omega$ and $\Psi$ are the operators defined in \eqref{Omega} and \eqref{Psi}.
Finally, for a matrix $K$ and for $n=0,1$, we define
\begin{align}
& \Phi(P_*,K,n) = Q^{\diamond}(n) + (K)^\tp R^{\diamond}(n)K
\notag\\
+ &(A^{\diamond}(n)+B^{\diamond}(n)K)^\tp \Pi(Y,n)(A^{\diamond}(n)+B^{\diamond}(n)K).
\label{Phi_2_def}
\end{align}
\end{definition}
We have the following lemma.
\begin{lemma}
For $n=0,1,$
\begin{small}
\begin{align}
\Omega^{\diamond}(P_*,n) = \Phi(P_*,\Psi^{\diamond}(P_*,n),n) = \min_K \Phi(P_*,K,n).
\label{eq:relation1}
\end{align}
\end{small}
Note that the minimization is in the sense of \red{partial order undefined?} $\succeq$, that is, the minimum value $\Omega^{\diamond}(P_*,n) \preceq \Phi(P_*,K,n)$ for all $K$.
\end{lemma}
\red{Proof}
\begin{lemma}
\begin{small}
\begin{align}
\Phi(P_*,K_*^0,0) = \Phi(P_*,\Psi^{\diamond}(P_*,0),0) = \Omega^{\diamond}(P_*,0) = P_*^0, \label{eq:claim1P0} \\
\Phi(P_*,\tilde K_*^1,1) = \Phi(P_*,\Psi^{\diamond}(P_*,1),1) = \Omega^{\diamond}(P_*,1) = P_*^1. \label{eq:claim1P1}
\end{align}
\end{small}
\end{lemma}
\red{Proof}

Now, using $\mathbb{T}_6$ and $\mathbb{T}_7$ calculated above and Definition \ref{def:Pi_2}, $\ee^{g^*}[V_{t+1}|H^0_t]$ can be written as,
\begin{align}
\ee^{g^*}[V_{t+1}|H^0_t]&= 
\hat X_{t+1|t} ^\tp \Pi(P_*,0) \hat X_{t+1|t}+  \tr (\Pi(P_*,1) \Sigma_{t+1|t}).
\label{V_t_1_2C}
\end{align}
%where we have used the definition of $\Pi(\cdot)$ in \eqref{Pi_matrix} where $\Theta$ is as defined in \eqref{eq:MJLS_theta}.

Note that \eqref{V_t_1_2C} involves  $\hat X_{t+1|t}$ and $\Sigma_{t+1|t}$. We will now try to write these in terms of  $\hat X_{t}$ and $\Sigma_{t}$. 
 For that purpose,  note that under the strategies $g^*$
\vspace{-2mm}
\begin{small}
\begin{align}
X_{t+1} &= AX_t + B \Big[ 
K_*^0\hat X_t + \bmat{\mathbf{0} \\ K_*^1 }(X_t - \hat X_t)
 \Big] + W_t \notag \\
& = A_s(0) \hat X_t + A_s(1)  ( X_t - \hat X_t) + W_t.
\label{X_dynamics_proof_2C}
\end{align}
\end{small}
In the above equation, we have defined $A_s(0) = A^{\diamond}(0) + B^{\diamond}(0) K_*^0$ and $A_s(1) = A^{\diamond}(1) + B^{\diamond}(1) \tilde K_*^1$ where  matrices $A^{\diamond}(m),B^{\diamond}(m)$, $m=0,1,$ are as defined in \eqref{eq:MJLS_A}-\eqref{eq:MJLS_B} and $\tilde K_*^1 =  \bmat{\mathbf{0} \\ K_*^1 }$. Now using \eqref{X_dynamics_proof_2C}, we can calculate $\hat X_{t+1|t}$ and $\Sigma_{t+1|t}$ as follows, 
\begin{align}
\label{estimation_X_2C}
&\hat X_{t+1|t} = A_s(0) \hat X_t, \\
&\Sigma_{t+1|t} =  \mathbf I + A_s(1) \Sigma_t A_s(1)^\tp.
\label{Sigma_t_2C}
\end{align}

\red{Many matrices are missing the diamonds, I have added some, but several remain....}

Using \eqref{estimation_X_2C}, we can write 
%\vspace{-4mm}
\begin{small}
\begin{align}
&\hat X_{t+1|t} ^\tp \Pi(P_*,0) \hat X_{t+1|t} \notag \\
& =\hat X_t ^\tp A_s(0)^\tp \Pi(P_*,0) A_s(0) \hat X_t
\notag\\
&= \hat X_t ^\tp \Big(\Phi(P_*,K_*^0,0) - Q(0) - (K_*^0)^\tp R(0) K_*^0 \Big)\hat X_t
\notag\\
&= \hat X_t^\tp P_*^0\hat X_{t}
 - \hat X_t^\tp Q(0) \hat X_{t}- (K_*^0\hat X_t)^\tp R(0) K_*^0\hat X_t
\label{eq:Vtp1_mean_2C}
\end{align}
\end{small}
where the first equality follows from the definition of $\Phi(P_*,K,0)$ in Definition \ref{def:Pi_2} and the second equality is correct because of \eqref{eq:claim1P0}.

%\vspace{-2mm}
%\begin{small}
%\begin{align}
%\Phi(P_*,K_*^0,0) = \Phi(P_*,\Psi^{\diamond}(P_*,0),0) = \Omega^{\diamond}(P_*,0) = P_*^0,
%\end{align}
%\end{small}
%where the first equality is true because from \eqref{eq:K_finite_2C_fixed}, $K_*^0 = \Psi^{\diamond}(P_*,0)$, the second equality is true from \eqref{eq:relation1} in Lemma \ref{lm:KPrelation}, and the last equality is true because of definition operator $\Omega^{\diamond}(\cdot)$ in \eqref{Omega_MJ} and \eqref{eq:P_finite_2C_fixed}.

Similarly, using \eqref{Sigma_t_2C}, we can write
\begin{small}
\begin{align}
&\tr (\Pi(P_*,1) \Sigma_{t+1|t})
\notag\\
&= \tr(\Pi(P_*,1)) + \tr((A_{s}(1))^\tp \Pi(P_*,1) A_{s}(1) \Sigma_t)
\notag\\
&= \tr(\Pi(P_*,1))
+\tr(\Phi(P_*,\tilde K_*^1,1) \Sigma_t)
\notag\\
&-\tr(Q(1)\Sigma_t)-\tr( (\tilde K_*^1)^\tp R(1) \tilde K_*^1 \Sigma_t)
\notag\\
&= \tr(\Pi(P_*,1))
+\tr(P_*^1 \Sigma_t)
\notag\\
&-\tr(Q(1) \Sigma_t)- \tr( (\tilde K_*^1)^\tp R(1) \tilde K_*^1 \Sigma_t),
\label{eq:Vtp1_variance_2C}
\end{align}
\end{small}
where the  first equality follows from the definition of $\Phi(P_*,K,1)$ in Definition \ref{def:Pi_2} and the second equality is correct because of \eqref{eq:claim1P1}.

Putting  \eqref{V_t_1_2C}, \eqref{eq:Vtp1_mean_2C} and \eqref{eq:Vtp1_variance_2C}together, we get
\begin{small}
\begin{align}
 \ee^{g^*}[V_{t+1}|H^0_t] &=  \hat X_t^\tp P_*^0\hat X_{t}
 - \hat X_t^\tp Q(0) \hat X_{t}- (K_*^0\hat X_t)^\tp R(0) K_*^0\hat X_t
 \notag \\
& + \tr(\Pi(P_*,1)) + \tr(P_*^1 \Sigma_t)
\notag\\
&-\tr(Q(1) \Sigma_t)- \tr( (\tilde K_*^1)^\tp R(1) \tilde K_*^1 \Sigma_t) \notag \\
&=  \tr(\Pi(P_*,1)) + \underbrace{\hat X_t^\tp P_*^0\hat X_{t} + \tr(P_*^1 \Sigma_t)}_{=V_t} \notag \\
& - \underbrace{[ \hat X_t^\tp Q(0)\hat X_t +\tr(Q(1) \Sigma_t)]}_{=\mathbb{T}_4} \notag \\
& -  \underbrace{[(K_*^0\hat X_t)^\tp R(0) K_*^0\hat X_t + \tr( (\tilde K_*^1)^\tp R(1) \tilde K_*^1 \Sigma_t)]}_{=\mathbb{T}_5}.
\label{eq:Vtp1_t_2C}
\end{align}
\end{small}

Adding \eqref{eq:Vtp1_t_2C} and \eqref{eq:calculated_c} and noting that $ \Pi(P_*,1) = \Lambda_*$ , we get 
%Since from \eqref{cost_given_h_2C}, $\ee[c(X_t,U_t^*)|H^0_t] = \mathbb{T}_4 + \mathbb{T}_5$ and furthermore, $ \tr(\Pi(P_*,1)) = \Lambda_*$, we have

\vspace{-3mm}
\begin{small}
\begin{align}
& \ee^{g^*}[V_{t+1}|H^0_t] + \ee^{g^*}[c(X_t,U_t^*)|H^0_t]
= \tr(\Lambda_*)
+ V_t ,
\end{align}
\end{small}
which proves \eqref{eq:main_goal_2C_2}.

==> old_proof_claim2.tex <==
\section{Proof of Claim \ref{claim:cost_optimal_NC}}
\label{Cost_of_the_Strategies}
\red{Start here}
We want to show that \eqref{eq:costforgstar_NC} holds. To this end, we show that 
\begin{align}
\ee [ c(X_t,U_t^*) | H_t^0]=  \tr(\Lambda_*)  + \ee [V_t - V_{t+1} | H_t^0].
\label{main_goal_NC}
\end{align}
where $\Lambda_* =  \sum_{n=1}^N \big( (1-p^n) [P_{*}^0]_{n,n}+p^n P_{*}^n \big)$.
Then, taking the expectation of the above equation and summing it from $0$ to $T$, the correctness of \eqref{eq:costforgstar_NC} is concluded as follows,
\begin{align}
J_{T}(g^*) 
= & \sum_{t=0}^T \ee [ c(X_t,U_t^*) ]
\notag\\
=&(T+1) \tr(\Lambda_*) 
+ \ee [V_0 - V_{T+1} ]
\notag\\
=&(T+1) \tr(\Lambda_*) 
- \ee [V_{T+1} ],
\end{align}
where the last equality holds because $V_0 = 0$. 

Now, to show that \eqref{main_goal_2C} holds, first note that $\ee[V_t | H_t^0] = V_t$ which is given by \eqref{V_t_2C}. Hence, we only need to calculate $\ee [ c(X_t,U_t^*) | H_t^0]$ and $\ee[V_{t+1} | H_t^0]$. 

\subsection{Calculating $\ee [ c(X_t,U_t^*) | H_t^0]$}
Note that 
\begin{small}
\begin{align}
&\ee [ c(X_t,U_t^*) | H_t^0]=  \underbrace{\ee [X_t^\tp Q X_t | H_t^0]}_{\mathbb{T}_4} + \underbrace{\ee[U_t^{*\tp} R U_t^* | H_t^0]}_{\mathbb{T}_5}. 
\label{cost_given_h}
\end{align}
\end{small}
We can simplify $\mathbb{T}_4$ as follows,
\begin{small}
\begin{align}
\mathbb{T}_4 &=  \hat X_t^\tp Q\hat X_t + \ee \Big[(X_t-\hat X_t)^\tp Q (X_t-\hat X_t)|H^0_t\Big] \notag \\
& =  \hat X_t^\tp Q\hat X_t + \sum_{n=1}^N \tr\big([Q]_{n,n}\Sigma_t^n \big) \notag \\
& =  \hat X_t^\tp Q(0)\hat X_t + \sum_{n=1}^N \tr\big([Q(n)]_{n,n}\Sigma_t^n \big),
\end{align}
\end{small}
where the second equality is correct because according to \cite[Lemma 3]{asghari_optimal_2017_arXiv},
given $H_t^0$, $X_t^n$ is independent of $X_t^m$ for $m \neq n$ and
the last equality is correct because from \eqref{Q_mj}, $Q(0) = Q$ and $[Q(n)]_{n,n} = [Q]_{n,n}= Q^{nn}$.
Similarly, since from \eqref{eq:opt_U_NC_fixed} we have $U_t^* = K_*^0 \hat X_t + \sum_{n=1}^N \tilde K_*^n (X_t - \hat X_t)$ where we have defined $\tilde K_*^n = \mathcal{L}_{zero}(K_*^0, K_*^n,n+1,n)$, we can simplify $\mathbb{T}_5$ as follows,

\vspace{-3mm}
\begin{small}
\begin{align}
\mathbb{T}_5 &=(K_*^0 \hat X_t)^\tp R K_*^0 \hat X_t +  \sum_{n=1}^N \tr \big( [(\tilde K_*^n)^{\tp} R \tilde K_*^n]_{n,n} \Sigma_{t}^n \big )
\notag\\
&= (K_*^0 \hat X_t)^\tp R(0) K_*^0 \hat X_t  
%\notag \\
%& 
+ \sum_{n=1}^N \tr \big( [(\tilde K_*^n)^{\tp} R(n) \tilde K_*^n]_{n,n} \Sigma_{t}^n \big ),
 \label{cost_on_U_t}
\end{align}
\end{small}
where the last equality is correct because from \eqref{R_mj}, $R(0) = R$ and $[(\tilde K_*^n)^{\tp} R \tilde K_*^n]_{n,n} = 
[(\tilde K_*^n)^{\tp} R(n) \tilde K_*^n]_{n,n} = (K_*^n)^{\tp} R^{nn} K_*^n$.

\subsection{Calculating $\ee[V_{t+1}|H^0_t]$}
For $n \in \mathcal{N}$, we define
\begin{align}
&\hat X_{t+1|t}^n := \ee [X_{t+1}^n|H^0_{t}]
\\
&\Sigma_{t+1|t}^n := \cov(X_{t+1}^n|H^0_{t})
 \\
&\Sigma_t^n := \cov(X_{t}^n|H^0_{t}).
\label{sigma_t}
\end{align}
Recall that $\hat{X}_t^n = \ee [X_{t}^n|H^0_{t}]$.  Note that under the strategies $g^*$ defined in \eqref{eq:costforgstar_NC} and from \eqref{Model:system}, we have 

\vspace{-2mm}
\begin{small}
\begin{align}
X_{t+1} &= AX_t + B \Big[ 
K_*^0\hat X_t +  \sum_{n=1}^N \tilde K_*^n (X_t - \hat X_t)
 \Big] + W_t \notag \\
& = A_s(0) \hat X_t + \sum_{n=1}^N A_s(n)  ( X_t - \hat X_t) + W_t.
\label{X_dynamics_proof_NC}
\end{align}
\end{small}
In the above equation, we have defined $A_s(0) = A(0) + B(0) K_*^0$ and $A_s(n) = A(n) + B(n) \tilde K_*^n$ for $n \in \mathcal{N}$ where  matrices $A(n),B(n)$, $n \in \overline{\mathcal{N}}$ are as defined in \eqref{A_mj}-\eqref{B_mj}. Note that the last equality of \eqref{X_dynamics_proof_NC} is correct because from \eqref{A_mj}-\eqref{B_mj}, $A(0) = A$, $\sum_{n=1}^N A(n) = A$, $B(0) =B$, and $B\tilde K_*^n = B(n) \tilde K_*^n$ for $n \in \mathcal{N}$. Now using \eqref{X_dynamics_proof_2C}, we can calculate $\hat X_{t+1|t}$ and $\Sigma^n_{t+1|t}$ as follows, 
\begin{align}
\label{estimation_X_NC}
&\hat X_{t+1|t} = A_s(0) \hat X_t \\
&\Sigma_{t+1|t}^n =  \mathbf I + [A_s(n)]_{n,n} \Sigma_t^n [A_s(n)]_{n,n}^\tp.
\label{Sigma_t_NC}
\end{align}
From the definition of $V_{t+1}$ in \eqref{V_t_NC} and considering \eqref{sigma_t}, we have

\vspace{-2mm}
\begin{small}
\begin{align}
& \ee[V_{t+1}|H^0_t]= \underbrace{\ee\Big[
\hat X_{t+1}^\tp P_*^0 \hat X_{t+1} \Big| H^0_t
\Big]}_{\mathbb{T}_6}
% \notag \\&
+ \underbrace{\ee\Big[
\sum_{n=1}^N \tr \big(P_*^n \Sigma_{t+1}^n \big )
\Big| H^0_t
\Big]}_{\mathbb{T}_7}.
\end{align}
\end{small}

Note that  when $\Gamma_{t+1}^n = 1$, $\hat X_{t+1}^n = X_{t+1}^n$ and hence $\Sigma_{t+1}^n = 0$. Further,  when $\Gamma_{t+1}^n = 0$, $\hat X_{t+1}^n = \hat X_{t+1|t}^n$ and $\Sigma_{t+1}^n = \Sigma_{t+1|t}^n$. Let $\Delta$ be a block diagonal matrix whose diagonal are block matrices $\Gamma_{t+1}^1 \mathbf{I}_{d_X^1}, \ldots, \Gamma_{t+1}^N \mathbf{I}_{d_X^N}$, that is,
\begin{align}
\Delta := \begin{bmatrix}
   \Gamma_{t+1}^1 \mathbf{I}_{d_X^1} & & \text{\huge0}\\
          & \ddots & \\
     \text{\huge0} & & \Gamma_{t+1}^N \mathbf{I}_{d_X^N}
\end{bmatrix}.
\label{Delta}
\end{align}
Note that $\Delta$ is a random matrix that depends on $\Gamma_{t+1}^1,\ldots,\Gamma_{t+1}^N$.
Then, we can write 
\begin{align}
\label{estimation_state}
&\hat X_{t+1} = \Delta X_{t+1} +(1-\Delta) \hat X_{t+1|t}, \\
 &\Sigma_{t+1}^n  = (1-\Gamma_{t+1}^n) \Sigma_{t+1|t}^n, \quad n \in \mathcal{N}.
\label{estimation_covariance}
\end{align}
Now, we use \eqref{estimation_state} and \eqref{estimation_covariance} to calculate $\mathbb{T}_6$ and $\mathbb{T}_7$.

\subsubsection{Calculating $\mathbb{T}_6$}
Note that from \eqref{estimation_state}, $\hat X_{t+1}$ can be written as $ \hat X_{t+1}= \hat X_{t+1|t} + \Delta (X_{t+1} -\hat X_{t+1|t})$. Considering this, $\mathbb{T}_6$ can be written as

\vspace{-2mm}
\begin{small}
\begin{align}
&\mathbb{T}_6= 
\ee\Big[
\hat X_{t+1|t} ^\tp P_*^0 \hat X_{t+1|t} \Big| H^0_t \Big] \notag \\
&+ \ee\Big[
(X_{t+1} -\hat X_{t+1|t})^\tp  \Delta^{\tp} P_*^0 \Delta (X_{t+1} -\hat X_{t+1|t}) \Big| H^0_t \Big] \notag \\ & = \hat X_{t+1|t} ^\tp P_*^0 \hat X_{t+1|t} + \sum_{n=1}^N (1-p^n) \tr \big ([P_*^0]_{n,n}  \Sigma_{t+1|t}^n  \big).
\label{T_4_1}
\end{align}
\end{small}

The last equality of \eqref{T_4_1} is correct because

\vspace{-2mm}
\begin{small}
\begin{align}
& \ee\Big[
(X_{t+1} -\hat X_{t+1|t})^\tp  \Delta^{\tp} P_*^0 \Delta (X_{t+1} -\hat X_{t+1|t}) \Big| H^0_t \Big] \notag \\ 
&= 
\ee\Big[ \ee[
(X_{t+1} -\hat X_{t+1|t})^\tp  \Delta^{\tp} P_*^0 \Delta (X_{t+1} -\hat X_{t+1|t}) 
%\notag \\
%&\hspace{6cm}  
| \Delta,H_t^0] \Big| H^0_t \Big] \notag \\ 
&= 
\ee\Big[ \sum_{n=1}^N
(X_{t+1}^n -\hat X_{t+1|t}^n)^\tp  [\Delta^{\tp} P_*^0 \Delta]_{n,n} (X_{t+1}^n -\hat X_{t+1|t}^n) 
%\notag \\
%&\hspace{6cm} 
\Big| H^0_t \Big] \notag \\ 
&= 
\sum_{n=1}^N \ee\Big[ 
(X_{t+1}^n -\hat X_{t+1|t}^n)^\tp (\Gamma_{t+1}^n)^2  [P_*^0]_{n,n} (X_{t+1}^n -\hat X_{t+1|t}^n) 
%\notag \\
%&\hspace{6cm} 
\Big| H^0_t \Big] \notag \\ 
&=  \sum_{n=1}^N (1-p^n) \tr \big ([P_*^0]_{n,n}  \Sigma_{t+1|t}^n  \big),
\label{T_4_1_1}
\end{align}
\end{small}
where the first equality is correct because of tower property and the second equality is correct because according to \cite[Lemma 3]{asghari_optimal_2017_arXiv}, given the common information $H_t^0$, $X_{t+1}^n$ is independent of $X_{t+1}^m$ for $m \neq n$. The third equality is correct because $[\Delta^{\tp} P_*^0  \Delta]_{n,n} = (\Gamma_{t+1}^n)^2  [P_*^0]_{n,n}$ which can be verified through straightforward algebraic manipulations by using \eqref{Delta}. Finally, the last equality is correct because each term of the summation is only non-zero when $\Gamma_{t+1}^n =1$ which happens with probability $1-p^n$.

\subsubsection{Calculating $\mathbb{T}_7$}
Considering \eqref{estimation_covariance}, it is straightforward to see that 

\vspace{-2mm}
\begin{small}
\begin{align}
&\mathbb{T}_7= \sum_{n=1}^N p^n \tr \big (P_*^n \Sigma_{t+1|t}^n  \big).
\end{align}
\end{small}

\subsubsection{Simplifying $\ee[V_{t+1}|H^0_t]$}
Now, using $\mathbb{T}_6$ and $\mathbb{T}_7$ calculated above, $\ee[V_{t+1}|H^0_t]$ can be written as,
\begin{align}
\ee[V_{t+1}|H^0_t]&= 
\hat X_{t+1|t} ^\tp \Pi(\tilde P_*^0,0) \hat X_{t+1|t} \notag \\
&+ \sum_{n=1}^N \tr \big ([\Pi(\tilde P_*^n,n)]_{n,n}  \Sigma_{t+1|t}^n  \big),
\label{V_t_1}
\end{align}
where we have defined $\tilde P_*^0 = P_*^0$ and $\tilde P_*^n = \mathcal{L}_{zero}(P_*^0, P_*^n,n,n)$. Further, we have used the fact that $[\tilde P_*^n]_{n,n} = P_*^n$ and the definition of $\Pi(\cdot)$ in \eqref{Pi_matrix} where $\Theta$ is as defined in \eqref{eq:MJLS_theta}.

Using \eqref{estimation_X_NC}, we can write $\hat X_{t+1|t} ^\tp \Pi(\tilde P_*,0) \hat X_{t+1|t}$ as follows,
%\vspace{-4mm}
\begin{small}
\begin{align}
& \hat X_t ^\tp A_s(0)^\tp \Pi(\tilde P_*,0) A_s(0) \hat X_t
\notag\\
&= \hat X_t ^\tp \Big(\Phi(\tilde P_*,K_*^0,0) - Q(0) - (K_*^0)^\tp R(0) K_*^0 \Big)\hat X_t
\notag\\
&= \hat X_t^\tp \tilde P_*^0\hat X_{t}
 - \hat X_t^\tp Q(0) \hat X_{t}- (K_*^0\hat X_t)^\tp R(0) K_*^0\hat X_t,
\label{eq:Vtp1_mean_NC}
\end{align}
\end{small}
where the first equality is true from \eqref{Phi_def} in Lemma \ref{lm:KPrelation}. Furthermore, the last equality is correct because

\vspace{-2mm}
\begin{small}
\begin{align}
\Phi(\tilde P_*,K_*^0,0) = \Phi(\tilde P_*,\Psi^{\diamond}(\tilde P_*,0),0) = \Omega^{\diamond}(\tilde P_*,0) = \tilde P_*^0,
\end{align}
\end{small}
where the first equality is true because from \eqref{eq:K_finite_2C_fixed}, $K_*^0 = \Psi^{\diamond}(\tilde P_*,0)$, the second equality is true from \eqref{eq:relation1} in Lemma \ref{lm:KPrelation}, and the last equality is true because of definition operator $\Omega^{\diamond}(\cdot)$ in \eqref{Omega_MJ} and \eqref{eq:P_finite_2C_fixed}.

Similarly, using \eqref{Sigma_t_NC} and by defining $\hat P_*^n = \Pi(\tilde P_*^n,n)$, $\tr \big ([\Pi(\tilde P_*^n,n)]_{n,n}  \Sigma_{t+1|t}^n  \big)$ can be written as
\begin{small}
\begin{align}
&\tr \big ([\Pi(\tilde P_*^n,n)]_{n,n}  \Sigma_{t+1|t}^n  \big)
\notag\\
&=\tr \big ([\hat P_*^n]_{n,n} \big) + \tr \big ([A_{s}(n)]_{n,n}^{\tp} [\hat P_*^n]_{n,n} [A_{s}(n)]_{n,n} \Sigma_t^n \big)
\notag\\
&= \tr \big ([\hat P_*^n]_{n,n} \big)  
+\tr(\Phi(\tilde P_*,\tilde K_*^n,n) \Sigma_t^n)
\notag\\
&-\tr \big( [Q(n)]_{n,n} \Sigma_t^n \big)-\tr \big( [(\tilde K_*^n)^\tp R(n) \tilde K_*^n]_{n,n} \Sigma_t^n \big)
\notag\\
&= \tr \big ([\hat P_*^n]_{n,n} \big)  
+\tr([\tilde P_*^n]_{n,n} \Sigma_t^n)
\notag\\
&-\tr \big( [Q(n)]_{n,n} \Sigma_t^n \big)- \tr \big( [(\tilde K_*^n)^\tp R(n) \tilde K_*^n]_{n,n} \Sigma_t^n \big).
\label{eq:Vtp1_variance_NC}
\end{align}
\end{small}
Putting \eqref{eq:Vtp1_mean_NC} and \eqref{eq:Vtp1_variance_NC} into \eqref{V_t_1} and using the fact that $[\tilde P_*^n]_{n,n} = P_*^n$, we get
\begin{small}
\begin{align}
& \ee[V_{t+1}|H^0_t]
\notag\\
& =  \hat X_t^\tp P_*^0\hat X_{t}
 - \hat X_t^\tp Q(0) \hat X_{t}- (K_*^0\hat X_t)^\tp R(0) K_*^0\hat X_t
 \notag \\
& + \sum_{n=1}^N \tr \big ([\hat P_*^n]_{n,n} \big) +\sum_{n=1}^N \tr(P_*^n \Sigma_t^n)
\notag\\
&- \sum_{n=1}^N \tr \big( [Q(n)]_{n,n} \Sigma_t^n \big)-  \sum_{n=1}^N \tr \big( [(\tilde K_*^n)^\tp R(n) \tilde K_*^n]_{n,n} \Sigma_t^n \big)
 \notag \\
&=\sum_{n=1}^N \tr \big ([\hat P_*^n]_{n,n} \big) + \underbrace{ \hat X_t^\tp P_*^0\hat X_{t} + \sum_{n=1}^N \tr(P_*^n \Sigma_t^n)}_{=V_t} \notag \\
& - \underbrace{[\hat X_t^\tp Q(0) \hat X_{t} + \sum_{n=1}^N \tr \big( [Q(n)]_{n,n} \Sigma_t^n \big)]}_{=\mathbb{T}_4} \notag \\
& - \underbrace{ [(K_*^0\hat X_t)^\tp R(0) K_*^0\hat X_t + \sum_{n=1}^N \tr \big( [(\tilde K_*^n)^\tp R(n) \tilde K_*^n]_{n,n} \Sigma_t^n \big)]
}_{=\mathbb{T}_5}.
\label{eq:Vtp1_t}
\end{align}
\end{small}

Note that from \eqref{cost_given_h}, we have $\ee[c(X_t,U_t^*)|H^0_t] = \mathbb{T}_4 + \mathbb{T}_5$ and furthermore, 

\vspace{-3mm}
\begin{small}
\begin{align}
&\sum_{n=1}^N [\hat P_*^n]_{n,n} = \sum_{n=1}^N [\Pi(\tilde P_*,n)]_{n,n} \notag \\
&= \sum_{n=1}^N \big( (1-p^n) [\tilde P_*^0]_{n,n} + p^n  [\tilde P_*^n]_{n,n} \big) \notag \\
&=
\sum_{n=1}^N \big( (1-p^n) [P_{*}^0]_{n,n}+p^n P_{*}^n \big) = \Lambda_*.
\end{align}
\end{small}

Therefore,
\begin{small}
\begin{align}
& \ee[V_{t+1}|H^0_t]
= \Lambda_*
+ V_t - \ee[c(X_t,U_t^*)|H^0_t],
\end{align}
\end{small}
which concludes the correctness of \eqref{main_goal_NC}.


==> proof_Lemma_10.tex <==
\section{Proof of Lemma \ref{lm:pc_NC}}
\label{proof_lm:pc}
The proof can be obtained by following a methodology similar to the one used to prove Lemma \ref{lm:pc_2C}. We can first use part 1 of Lemma \ref{lm:ss} to show that the auxiliary MJLS described by \eqref{A_mj}-\eqref{transition_prob} is SS if and only if $p^n < p_c^n$ for all $n \in \mathcal{N}$ where $p_c^n$ is the critical threshold given by \eqref{eq:pc}. 

Second, we can use part 2 of Lemma \ref{lm:ss} to show that the auxiliary MJLS described by \eqref{A_mj}-\eqref{transition_prob} is SD if and only of $\mathcal{A}_d$ defined as in \eqref{eq:bigmatrix3} is Schur stable. Since the matrix $\mathcal{A}_{d}$ is upper-triangular, it is Schur stable if and only if there exist matrices $H^{\diamond}(0)$ and $H^{\diamond}(n)$ for $n \in \mathcal{N}$ such that $\rho\big(A_d(0)\otimes A_d(0)\big)<1$ and $\rho\big(p^n A_d(n)\otimes A_d(n)\big)<1$ where $A_d(n)$, $n \in \mathcal{N}$, defined as in \eqref{A_c_l}. The existence of these matrices is resulted since $(A,Q)$ and $\big(A^{nn},(Q^{nn})^{1/2} \big)$ for all $n \in \mathcal{N}$ are detectable from Assumptions \ref{assum:det_stb} and \ref{assum:det_stb_2}. %, there exist matrices $H^{\diamond}(0)$ and $H^{\diamond}(n)$ for $n \in \mathcal{N}$ such that $\rho\big(A_d(0)\otimes A_d(0)\big)<1$ and $\rho\big(p^n A_d(n)\otimes A_d(n)\big)<1$. 
Hence, the MJLS is SD.

It then follows from Lemma \ref{lm:MJ_infinite} that matrices $P^{\diamond}_{t}(n)$, $n \in \overline{\mathcal{N}}$, converge as $t \to -\infty$ to PSD matrices $P^{\diamond}_{*}(n)$ that satisfy the steady state version of \eqref{P_MJ_cmp_NC_0}-\eqref{P_MJ_cmp_NC_1} (i.e., equations \eqref{eq:P_finite_NC_fixed}-\eqref{eq:tildeP_finite_NC_fixed}) if and only if $p^n < p_c^n$ for all $n \in \mathcal{N}$. This proves the lemma.

\begin{figure*}[t]
\begin{small}
\begin{align}
\mathcal{A}_d =
\begin{blockarray}{ccccc}
\begin{block}{[ccccc]}
                     A_d(0)\otimes A_d(0) & (1-p^1)A_d(1)\otimes A_d(1)& (1-p^2)A_d(2)\otimes A_d(2) & \ldots & (1-p^n)A_d(N)\otimes A_d(N) \\ \\
                     \mathbf{0} & p^1A_d(1)\otimes A_d(1) &\mathbf{0} &\ldots & \mathbf{0} \\ \\
                     \vdots &\ddots  &p^2 A_d(2)\otimes A_d(2)  & \ddots & \vdots \\ \\
                     \vdots &   &\ddots  &\ddots & \mathbf{0} \\ \\
                     \mathbf{0} & \ldots &\ldots & \mathbf{0}  & p^n A_d(N)\otimes A_d(N)\\
\end{block}
\end{blockarray}
\label{eq:bigmatrix3}
\end{align}
\end{small}
\hrule
\end{figure*}
\begin{figure*}[t]
\begin{small}
\begin{align}
&A_d(n) = A^{\diamond} (n) +  H^{\diamond}(n) \big(Q^{\diamond}(n) \big)^{1/2}
= \begin{blockarray}{cccl}
\text{$1:n-1$} &n &\text{$n+1:N$}  &  \\
\begin{block}{[ccc]l}
                      \text{\large 0}   & [H^{\diamond}(n)]_{n,1:n-1} (Q^{nn})^{1/2} &\text{\large 0} & \text{$1:n-1$} \\
   \text{\large 0} & A^{nn} + [H^{\diamond}(n)]_{n,n} (Q^{nn})^{1/2} & \text{\large 0} &n \\
                      \text{\large 0}   & [H^{\diamond}(n)]_{n,n+1:N} (Q^{nn})^{1/2} & \text{\large 0}&\text{$n+1:N$}  \\
\end{block}
\end{blockarray}.
\label{A_c_l}
\end{align}
\end{small}
\hrule
\end{figure*} 

==> proof_Lemma_12.tex <==
{\color{blue}
\section{Proof of Lemma \ref{lm:opt_strategies_new_rep}}
\label{proof_lm:opt_strategies_new_rep}
By comparing \eqref{eq:P_N_init}-\eqref{eq:P_finite} with  \eqref{eq:barP_init}-\eqref{eq:barP_finite_0}, it is straightforward to observe that $P_t^0 = \bar P_t^0$ for all $t$. We will now show by induction that at any time $t$, $P_t^n = \bar P_t^n$ for $n =1,\ldots,N$.
First note that by definition, $P_{T+1}^{n} = \mathbf{0}$ and $\bar P^n_{T+1} = \mathbf{0}$ for $n =1,\ldots,N$. Hence, \eqref{new_rep2} is correct at time $T+1$. Now, assume that \eqref{new_rep2} is correct at time $t+1$ (induction hypothesis). Then, from \eqref{eq:barP_finite} and  the induction hypothesis, we have for $n =1,\ldots,N$,
\begin{align}
\bar P_t^{n} &=  \Omega \big((1-p^n) P_{t+1}^0+p^n \mathcal{L}_{zero}(P^0_{t+1}, P_{t+1}^{n},n,n), \notag \\
& \hspace{1.0cm}  \mathcal{L}_{zero}(Q,Q^{nn},n,n), \mathcal{L}_{iden}(R,R^{nn},n+1), \notag \\
 & \hspace{1.0cm}  \mathcal{L}_{zero}(A,A^{nn},n,n), \mathcal{L}_{zero}(B,B^{nn},n,n+1) \big) \notag \\
&=
\mathcal{L}_{zero}(Q,Q^{nn},n,n)  + \mathbb{T}_1 - \mathbb{T}_2 (\mathbb{T}_3)^{-1} (\mathbb{T}_2)^{\tp},
\label{P_MJ_n}
\end{align}
where 
\begin{align}
\label{T_1_def}
&\mathbb{T}_1 = \mathcal{L}_{zero}(A,A^{nn},n,n)^{\tp} \bar{\bar{P}}_{t+1} \mathcal{L}_{zero}(A,A^{nn},n,n) \\
\label{T_2_def}
&\mathbb{T}_2 = \mathcal{L}_{zero}(A,A^{nn},n,n)^{\tp} \bar{\bar{P}}_{t+1} \mathcal{L}_{zero}(B,B^{nn},n,n+1) , \\
\label{T_3_def}
&\mathbb{T}_3 = \mathcal{L}_{iden}(R,R^{nn},n+1) 
\notag \\
&+ \mathcal{L}_{zero}(B,B^{nn},n,n+1)^{\tp} \bar{\bar{P}}_{t+1} \mathcal{L}_{zero}(B,B^{nn},n,n+1),
\end{align}
and we have defined $\bar{\bar{P}}_{t+1} = (1-p^n) P_{t+1}^0+p^n \mathcal{L}_{zero}(P^0_{t+1}, P_{t+1}^{n},n,n)$.

Note that from the definitions of operators $\mathcal{L}_{zero}$ and $\mathcal{L}_{iden}$ in \eqref{L_zero}-\eqref{L_iden}, it is straightforward to observe that the block dimensions of $\mathbb{T}_1, \mathbb{T}_2, \mathbb{T}_3$ are the same as the block dimensions of $A,B,B^{\tp} B$, respectively (They are block matrices of sizes $N \times N$, $N \times (N+1)$, and $(N+1) \times (N+1)$, respectively). Therefore, through straightforward algebraic manipulations, we can get
\begin{align}
\label{T_1}
&\mathbb{T}_1 = \mathcal{L}_{zero}(A,\mathbb{\tilde T}_1,n,n), \\
\label{T_2}
&\mathbb{T}_2 =  \mathcal{L}_{zero}(B,\mathbb{\tilde T}_2,n,n+1), \\
\label{T_3}
&\mathbb{T}_3 = \mathcal{L}_{iden}(B^{\tp}B,\mathbb{\tilde T}_3,n+1),
\end{align}
where
\begin{align}
\label{tilde_T_1}
&\mathbb{\tilde T}_1 = (A^{nn})^{\tp}[(1-p^n)[P_{t+1}^0]_{n,n}+p^n P_{t+1}^{n}]A^{nn}, \\
\label{tilde_T_2}
&\mathbb{\tilde T}_2 = (A^{nn})^{\tp}[(1-p^n)[P_{t+1}^0]_{n,n}+p^n P_{t+1}^{n}]B^{nn}, \\
\label{tilde_T_3}
&\mathbb{\tilde T}_3 = R^{nn} + (B^{nn})^{\tp}[(1-p^n)[P_{t+1}^0]_{n,n}+p^n P_{t+1}^{n}]B^{nn}.
\end{align}

Further, since $\mathbb{T}_3$ is a block diagonal matrix, we have 
\begin{align}
& (\mathbb{T}_3)^{-1} =\mathcal{L}_{iden} \big(B^{\tp}B,(\mathbb{\tilde T}_3)^{-1},n+1 \big).
\label{T_3_inv}
\end{align}

Now, using \eqref{T_1}-\eqref{T_3_inv} and the fact that  matrices $A, Q, BB^{\tp}$ have the same size as matrix $P^0_t$ (They are block matrices of size $N \times N$), \eqref{P_MJ_n} can be simplified to
\begin{align}
\bar P_t^{n} &= \mathcal{L}_{zero} \big(P^0_t,  Q^{nn} + \mathbb{\tilde T}_1 - \mathbb{\tilde T}_2 (\mathbb{\tilde T}_3)^{-1} (\mathbb{\tilde T}_2)^{\tp},n,n \big) \notag \\
&=   \mathcal{L}_{zero}(P^0_t, P_t^{n},n,n),
\end{align}
where the last equality is true because of the definition of $P_t^{n}$ in \eqref{eq:tildeP_finite}. Hence, \eqref{new_rep2} is true at time $t$. This completes the proof.
}


{\color{blue}
\section{Proof of Lemma \ref{lm:pc_NC}}
\label{proof_lm:pc}
From Lemma \ref{lm:opt_strategies_new_rep}, we know that the convergence of matrices $P_t^{n}$, $n \in \mathcal{\overline N}$, is equivalent to the convergence of matrices $\bar P_t^{n}$, $n \in \mathcal{\overline N}$. Further, because of Lemma \ref{equality_recursions_NC}, $\bar P^n_t = P^{\diamond}_t(n)$, $n \in \mathcal{\overline N}$, where matrices $P^{\diamond}_t(n)$, $n \in \mathcal{\overline N}$, are defined by \eqref{eq:P_N_MJ_init}-\eqref{P_MJ_cmp_NC_1} for the auxiliary MJLS. Thus, in order to study the the convergence of matrices $P_t^{n}$, $n \in \mathcal{\overline N}$, we can focus on the convergence of matrices $P^{\diamond}_t(n)$, $n \in \mathcal{\overline N}$.

To investigate the convergence of $P^{\diamond}_t(n)$, $n \in \mathcal{\overline N}$, we can follow a methodology similar to the one used to prove Lemma \ref{lm:pc_2C}. We first use part 1 of Lemma \ref{lm:ss} to show that the auxiliary MJLS described by \eqref{A_mj}-\eqref{transition_prob} is SS if and only if $p^n < p_c^n$ for all $n \in \mathcal{N}$ where $p_c^n$ is the critical threshold given by \eqref{eq:pc}. 

Second, we can use part 2 of Lemma \ref{lm:ss} to show that the auxiliary MJLS described by \eqref{A_mj}-\eqref{transition_prob} is SD if and only of $\mathcal{A}_d$ defined as in \eqref{eq:bigmatrix3} is Schur stable. Since the matrix $\mathcal{A}_{d}$ is upper-triangular, it is Schur stable if and only if there exist matrices $H^{\diamond}(0)$ and $H^{\diamond}(n)$ for $n \in \mathcal{N}$ such that $\rho\big(A_d(0)\otimes A_d(0)\big)<1$ and $\rho\big(p^n A_d(n)\otimes A_d(n)\big)<1$ where $A_d(n)$, $n \in \mathcal{N}$, defined as in \eqref{A_c_l}. The existence of these matrices is resulted since $(A,Q)$ and $\big(A^{nn},(Q^{nn})^{1/2} \big)$ for all $n \in \mathcal{N}$ are detectable from Assumptions \ref{assum:det_stb} and \ref{assum:det_stb_2}. %, there exist matrices $H^{\diamond}(0)$ and $H^{\diamond}(n)$ for $n \in \mathcal{N}$ such that $\rho\big(A_d(0)\otimes A_d(0)\big)<1$ and $\rho\big(p^n A_d(n)\otimes A_d(n)\big)<1$. 
Hence, the MJLS is SD.

It then follows from Lemma \ref{lm:MJ_infinite} that matrices $P^{\diamond}_{t}(n)$, $n \in \overline{\mathcal{N}}$, converge as $t \to -\infty$ to PSD matrices $P^{\diamond}_{*}(n)$ that satisfy the steady state version of \eqref{P_MJ_cmp_NC_0}-\eqref{P_MJ_cmp_NC_1} (i.e., equations \eqref{eq:P_finite_NC_fixed}-\eqref{eq:tildeP_finite_NC_fixed}) if and only if $p^n < p_c^n$ for all $n \in \mathcal{N}$. This proves the lemma.

\begin{figure*}[t]
\begin{small}
\begin{align}
\mathcal{A}_d =
\begin{blockarray}{ccccc}
\begin{block}{[ccccc]}
                     A_d(0)\otimes A_d(0) & (1-p^1)A_d(1)\otimes A_d(1)& (1-p^2)A_d(2)\otimes A_d(2) & \ldots & (1-p^n)A_d(N)\otimes A_d(N) \\ \\
                     \mathbf{0} & p^1A_d(1)\otimes A_d(1) &\mathbf{0} &\ldots & \mathbf{0} \\ \\
                     \vdots &\ddots  &p^2 A_d(2)\otimes A_d(2)  & \ddots & \vdots \\ \\
                     \vdots &   &\ddots  &\ddots & \mathbf{0} \\ \\
                     \mathbf{0} & \ldots &\ldots & \mathbf{0}  & p^n A_d(N)\otimes A_d(N)\\
\end{block}
\end{blockarray}
\label{eq:bigmatrix3}
\end{align}
\end{small}
\hrule
\end{figure*}
\begin{figure*}[t]
\begin{small}
\begin{align}
&A_d(n) = A^{\diamond} (n) +  H^{\diamond}(n) \big(Q^{\diamond}(n) \big)^{1/2}
= \begin{blockarray}{cccl}
\text{$1:n-1$} &n &\text{$n+1:N$}  &  \\
\begin{block}{[ccc]l}
                      \text{\large 0}   & [H^{\diamond}(n)]_{n,1:n-1} (Q^{nn})^{1/2} &\text{\large 0} & \text{$1:n-1$} \\
   \text{\large 0} & A^{nn} + [H^{\diamond}(n)]_{n,n} (Q^{nn})^{1/2} & \text{\large 0} &n \\
                      \text{\large 0}   & [H^{\diamond}(n)]_{n,n+1:N} (Q^{nn})^{1/2} & \text{\large 0}&\text{$n+1:N$}  \\
\end{block}
\end{blockarray}.
\label{A_c_l}
\end{align}
\end{small}
\hrule
\end{figure*} 
}

==> stability_proof.tex <==
\section{Proof of Lemma \ref{lm:Q2_2C}, part 3}\label{sec:stability_proof}
 Let $\tilde X_t := X_t - \hat X_t$ denote the  estimation error.  It suffices to show that $\hat X_t$ and  $\tilde X_t$ are mean square stable.

The optimal strategies can be written as 
\begin{align}
U_t = K^0_* \hat X_t + 
\begin{bmatrix}
0 \\ K^1_* 
\end{bmatrix}
\tilde X_t.
\end{align}
%Note that the estimate is given by
%\begin{align}
%&\hat X_{t+1} 
%\notag\\
%= &\Gamma_{t+1} X_{t+1}
% + ( 1 - \Gamma_{t+1})(A + B K^0_* ) \hat X_t
% \notag\\
% = &\Gamma_{t+1}
%(A X_t + B U_t + W_t)
% + ( 1 - \Gamma_{t+1})(A + B K^0_* ) \hat X_t
% \notag\\
% = & (A + B K^0_* ) \hat X_t + \Gamma_{t+1}((A + B^{11}K^1_*) \tilde X_t + W_t))
%\end{align}
%and the remaining part is given by
%\begin{align}
%&\tilde X_{t+1} 
%\notag\\
%= &(1-\Gamma_{t+1}) (X_{t+1} -(A + B K^0_* ) \hat X_t)
% \notag\\
% = & (1-\Gamma_{t+1})((A + B^{11}K^1_*) \tilde X_t + W_t))
%\end{align}
%From the above equations, the dynamics of the closed-loop system can be described as

After some algebra, the   closed-loop dynamics of $(\hat X_t, \tilde X_t)$ under the optimal strategies can be written as
\begin{align}
\begin{bmatrix}
\hat X_{t+1}\\
\tilde X_{t+1}
\end{bmatrix}
= 
A_{cl}(\Gamma^1_{t+1})
\begin{bmatrix}
\hat X_{t} \\
\tilde X_{t} 
\end{bmatrix}
+ G_{cl}(\Gamma^1_{t+1}) W_t,
\end{align}
where
\begin{small}
\begin{align}
A_{cl}(\Gamma^1_{t+1}) = &
\begin{bmatrix}
(A + B K^0_* ) & \Gamma^1_{t+1}(A + B^{11}K^1_*) \\
0 & (1-\Gamma^1_{t+1})(A + B^{11}K^1_*) 
\end{bmatrix},
\\
G_{cl}(\Gamma^1_{t+1}) = &
\begin{bmatrix}
\Gamma^1_{t+1}
\\
(1-\Gamma^1_{t+1})
\end{bmatrix},
\end{align}
\end{small}
and $\hat X_0 =0, \tilde X_0=0$.

If $p^1 = 0$ or $1$, the stability result follows from standard  linear system theory arguments.
If $0< p^1 < 1$, the closed-loop system is a MJLS with an i.i.d. switching process\footnote{Note that this MJLS is not the same as the auxiliary MJLS constructed in Section \ref{sec:Q1_2C}.}.
From \cite[Theorem 3.33]{costa2006discrete}, the closed-loop system is mean square stable if the corresponding  noiseless system (i.e., with $W_t = 0$) is mean square stable.
Because $\Gamma_{t+1}^1$ is an i.i.d. process, from \cite[Corollary 2.7]{fang2002stochastic}, the noiseless system is mean-square stable if
the spectral radius of the matrix
\begin{align}\label{eq:ms_eq1}
& p^1 A_{cl}(0) \otimes A_{cl}(0)+ (1 - p^1) A_{cl}(1) \otimes A_{cl}(1) =
\notag\\
&
\begin{tiny}
\begin{bmatrix} 
A_s(0) \otimes 
\begin{bmatrix}
A_s(0) & (1-p^1)A_s(1)\\
 \mathbf{0} & p^1 A_s(1)
\end{bmatrix}
& 
(1-p^1) A_s(1) \otimes 
\begin{bmatrix}
A_s(0) & A_s(1)\\
 \mathbf{0} &  \mathbf{0}
\end{bmatrix}
\\
 \mathbf{0}
&
p^1 A_s(1) \otimes 
\begin{bmatrix}
A_s(0) &  \mathbf{0}\\
 \mathbf{0} & A_s(1)
\end{bmatrix}
\end{bmatrix}
\end{tiny}
\end{align}
is less than one, where $A_s(0) = (A + B K^0_* )$ and $A_s(1) = (A + B^{11}K^1_*)$.
%Since $(A,B)$ is stabilizable, $\rho(A + B K^0_* ) < 1$. Then, from the matrix's block structure, its spectral radius is bounded by $\max(1,p^1(\rho( A_s(1)))^2)$. Consequently, it remains to show that $\rho(p^1 A_s(1) \otimes A_s(1)) < 1$.


Note that the gain matrices $K^0_* ,K^1_* $ are obtained from the CARE in \eqref{eq:CARE_infinite} for the SD and SS auxiliary MJLS described by \eqref{eq:MJLS_A}-\eqref{eq:MJLS_theta}, so the corresponding gains stabilize the auxiliary MJLS \cite[Corollary A.16]{costa2006discrete}, \cite[Theorem A.15]{costa2006discrete}. That is, the following matrix
\begin{align}
\mathcal{A}_s = \begin{bmatrix}
A_s(0)\otimes A_s(0) & (1-p^1)A_s(1)\otimes A_s(1) \\
 \mathbf{0} & p^1A_s(1)\otimes A_s(1)
\end{bmatrix}
\end{align}
has a spectral radius less than one (see the proof of Lemma \ref{lm:pc_2C}). Thus, $\rho(A_s(0)) < 1$ and $\rho(A_s(1)) <  \frac{1}{\sqrt p^1}$. Consequently, the spectral radius of the matrix in \eqref{eq:ms_eq1} is less than $1$. This establishes the mean-square stability of $(\hat X_t, \tilde X_t)$.



%\blue{Stability result}
%
%\red{TO BE EDITED}
%
%\begin{lemma}
%If $p^1 < p^1_c$, the closed-loop system under the optimal strategies is mean-square stable in the sense that
%$\ee[X_t] \rightarrow EX$ and $\ee[ ||X_t||^2] \rightarrow EX^2$ where $EX$ and $EX^2$ are finite numbers.
%\end{lemma}
%\begin{proof}
%Let $\tilde X_t = X_t - \hat X_t$ be the remaining part of the state minus the estimate. 
%Then, the optimal strategies are given by
%\begin{align}
%U_t = K^0_* \hat X_t + 
%\begin{bmatrix}
%0 \\ K^1_* 
%\end{bmatrix}
%\tilde X_t
%\end{align}
%Note that the estimate is given by
%\begin{align}
%&\hat X_{t+1} 
%\notag\\
%= &\Gamma_{t+1} X_{t+1}
% + ( 1 - \Gamma_{t+1})(A + B K^0_* ) \hat X_t
% \notag\\
% = &\Gamma_{t+1}
%(A X_t + B U_t + W_t)
% + ( 1 - \Gamma_{t+1})(A + B K^0_* ) \hat X_t
% \notag\\
% = & (A + B K^0_* ) \hat X_t + \Gamma_{t+1}((A + B^{11}K^1_*) \tilde X_t + W_t))
%\end{align}
%and the remaining part is given by
%\begin{align}
%&\tilde X_{t+1} 
%\notag\\
%= &(1-\Gamma_{t+1}) (X_{t+1} -(A + B K^0_* ) \hat X_t)
% \notag\\
% = & (1-\Gamma_{t+1})((A + B^{11}K^1_*) \tilde X_t + W_t))
%\end{align}
%
%From the above equations, the dynamics of the closed-loop system can be described as
%\begin{align}
%\begin{bmatrix}
%\hat X_{t+1}\\
%\tilde X_{t+1}
%\end{bmatrix}
%= 
%A_{cl}(\Gamma_{t+1})
%\begin{bmatrix}
%\hat X_{t} \\
%\tilde X_{t} 
%\end{bmatrix}
%+ G_{cl}(\Gamma_{t+1}) W_t
%\end{align}
%where
%\begin{align}
%A_{cl}(\Gamma_{t+1}) = &
%\begin{bmatrix}
%(A + B K^0_* ) & \Gamma_{t+1}(A + B^{11}K^1_*) \\
%0 & (1-\Gamma_{t+1})(A + B^{11}K^1_*) 
%\end{bmatrix}
%\\
%G_{cl}(\Gamma_{t+1}) = &
%\begin{bmatrix}
%\Gamma_{t+1}
%\\
%(1-\Gamma_{t+1})
%\end{bmatrix}
%\end{align}
%Therefore, the closed-loop system is a MJLS.
%From \cite[Theorem 3.33]{costa2006discrete}, the closed-loop system is mean-square stable if the noiseless system (i.e., $W_t = 0$) is mean-square stable.
%Because $\Gamma_{t+1}$ is an i.i.d. process, from \cite{fang2002stochastic}, the noiseless system is mean-square stable if
%the spectral radius of the matrix
%
%\begin{align}
%& p^1 A_{cl}(0) \otimes A_{cl}(0)+ (1 - p^1) A_{cl}(1) \otimes A_{cl}(1) =
%\notag\\
%&
%\begin{tiny}
%\begin{bmatrix} 
%A_s(0) \otimes A_s(0)  & \bar p^1A_s(0) \otimes A_s(1) & \bar p^1 A_s(1) \otimes A_s(0) & \bar p^1 A_s(1) \otimes A_s(1) \\
%0 & p^1 A_s(0)\otimes A_s(1)  & 0 & 0 \\
%0 & 0 & p^1 A_s(1) \otimes A_s(0) & 0\\
%0 & 0 & 0 & p^1 A_s(1) \otimes A_s(1)
%\end{bmatrix}
%\end{tiny}
%\end{align}
%is less than one, where $\bar p^1 = 1 - p^1$, $A_s(0) = (A + B K^0_* )$ and $A_s(1) = (A + B^{11}K^1_*)$.
%Since $(A,B)$ is stabilizable, $\rho(A + B K^0_* ) < 1$. Then, from the matrix's block structure, it remains to show that $\rho(p^1 A_s(1) \otimes A_s(1)) < 1$.
%
%
%Note that the optimal strategies are obtained from the CARE \eqref{eq:CARE_infinite}, so the corresponding gains stabilize the auxiliary MJLS described by \eqref{eq:MJLS_A}-\eqref{eq:MJLS_theta}. That is, the following matrix
%\begin{align}
%\mathcal{A}_s = \begin{bmatrix}
%A_s(0)\otimes A_s(0) & (1-p^1)A_s(1)\otimes A_s(1) \\
% \mathbf{0} & p^1A_s(1)\otimes A_s(1)
%\end{bmatrix}
%\end{align}
%has a spectral radius less than one (see the proof of Lemma \ref{lm:pc_2C}). Consequently, $\rho(p^1 A_s(1) \otimes A_s(1)) < 1$ and we establish the mean-square stability of the closed-loop system.
%\end{proof}


==> timeline.tex <==
\begin{figure}[h]
\begin{center}
\begin{tikzpicture}[node distance=1cm]
\draw [thick,->,>=stealth,line width=1pt] (1,1) -- (8,1) node[right]{time};
\draw [thick] (1.5,1) -- (1.5,0.9) node[below] {$t$};
\draw [thick] (7,1) -- (7,0.9) node[below] {$t+1$};

\draw [thick,->,>=stealth,line width=1pt] (1,0) -- (8,0) node[right]{time};
\draw [thick] (1.5,0) -- (1.5,-0.1) node[below] {$t$};
\draw [thick] (7,0) -- (7,-0.1) node[below] {$t+1$};

%\node (Nat) at (0,2) {Nature};

\node (Xt) at (2,1.3) {$X_t^n$};
\draw (2,1) node[cross=2.5pt] {};

\node (Gamt) at (3,1.3) {$\Gamma_t^n$};
\draw (3,1) node[cross=2.5pt] {};

%\node (Gamt) at (2.5,0.3) {$\Gamma_t^{1:N}$};
%\draw (2.5,0) node[cross=2.5pt] {};

\node (Zt) at (4,1.3) {$Z_t^n$};
\draw (4,1) node[cross=2.5pt] {};

\node (Zt) at (4,0.3) {$Z_t^{1:N}$};
\draw (4,0) node[cross=2.5pt] {};

%\node (HtR) at (4,1.3) {$H_t^0$};
%\draw (4,1) node[cross=2.5pt] {};
%
%\node (HtR) at (4,0.3) {$H_t^0$};
%\draw (4,0) node[cross=2.5pt] {};
%
%\node (HtL) at (4.7,1.3) {$H_t^{n}$};
%\draw (4.7,1) node[cross=2.5pt] {};

\node (UtL) at (5.5,1.3) {$U_t^{n}$};
\draw (5.5,1) node[cross=2.5pt] {};

\node (UtL) at (5.5,0.3) {$U_t^{0}$};
\draw (5.5,0) node[cross=2.5pt] {};

\node (Wt) at (6.5,1.3) {$W_t^{n}$};
\draw (6.5,1) node[cross=2.5pt] {};

\node (Xtp) at (7.5,1.3) {$X_{t+1}^n$};
\draw (7.5,1) node[cross=2.5pt] {};


\node (CL) at (.5,1) {$C^{n}$} ;
\node (CR) at (.5,0) {$C^0$} ;

%\node (C) at (1.5,-1) {$C$} ;


\end{tikzpicture}
\caption{Time-ordering of relevant variables.}
\label{fig:timing}

\end{center}
\end{figure}
